Topics of Concern: Identifying User Issues in Reviews of IoT Apps and Devices

Internet of Things (IoT) systems are bundles of networked sensors and actuators that are deployed in an environment and act upon the sensory data that they receive. These systems, especially consumer electronics, have two main cooperating components: a device and a mobile app. The unique combination of hardware and software in IoT systems presents challenges that are lesser known to mainstream software developers. They might require innovative solutions to support the development and integration of such systems. In this paper, we analyze more than 90,000 reviews of ten IoT devices and their corresponding apps and extract the issues that users encountered while using these systems. Our results indicate that issues with connectivity, timing, and updates are particularly prevalent in the reviews. Our results call for a new software-hardware development framework to assist the development of reliable IoT systems.

==> data.tex <==
\section{Data}

% In this section we describe what is our data source, how we selected them, how we extracted them.

Our data came from the Google Play Store. Each app has its own page that displays the app information, including screenshots of the app in use, a description of the app's purpose and functionality, and a list of reviews left by users of the app. These user reviews were the point of interest for this paper.

%% Why do we choose this apps?

We wanted to look specifically at apps that were a part of the Internet of Things. Based off our own searching, we included apps in our study that appeared to be some of the most popular IoT apps. Some apps, such as Kevo, were not as widely used, but we included them, because previous studies on app reviews had included them. We included those apps as well to see how our data compared with prior data.

%%How we extract the data from Google Play

We created a program written in Python using the Selenium library to crawl the reviews on each app page.The program would access each review, starting with the first one displayed on the page and extract the following information

% per App we need to explain following info
%% What are the characteristics of data: time (first review to last review),
%% number of users 
